Indeterministic finite-precision physics and intuitionistic mathematics

In recent publications in physics and mathematics, concerns have been raised about the use of real numbers to describe quantities in physics, and in particular about the usual assumption that physical quantities are infinitely precise. In this thesis, we discuss some motivations for dropping this assumption, which we believe partly arises from the usual point-based approach to the mathematical continuum. We focus on the case of classical mechanics specifically, but the ideas could be extended to other theories as well. We analyse the alternative theory of classical mechanics presented by Gisin and Del Santo, which suggests that physical quantities can equivalently be thought of as being only determined up to finite precision at each point in time, and that doing so naturally leads to indeterminism. Next, we investigate whether we can use intuitionistic mathematics to mathematically express the idea of finite precision of quantities, arriving at the cautious conclusion that, as far as we can see, such attempts are thwarted by conceptual contradictions. Finally, we outline another approach to formalising finite-precision quantities in classical mechanics, which is inspired by the intuitionistic approach to the continuum but uses classical mathematics.

==> chapters/entropy-information.tex <==
\chapter{Entropy and information}

\lettrine[lines=3]{T}{hrough the ages,} many notions of entropy have been introduced. While they are similar in some ways and therefore all go by the same name, they differ in others, creating a notorious source of confusion. The relation between entropy and information, in particular, is complicated and hence often misrepresented.

In this section, I will briefly introduce some notions of entropy and explain their relation to the notion of information, and draw some conclusions about the relation between information theory and physical entropy. This is far from a comprehensive treatment. See e.g. \textcite{FrW11} for a more complete overview of different notions of entropy and their relations. \textcite{Cat08} focuses on the relation with information. There has also been a lot of thought on the connections between (algorithmic) information theory and entropy in statistical mechanics, notably in the work of Jaynes (see references in \textcite{FrW11}) and more recently \textcite{tadaki2019}, and information theory and thermodynamic entropy, by Brillouin and Landauer \cite{sep-information-entropy}. I will also briefly introduce Bekenstein’s bound, which will be the subject of section~\ref{sec:...}.

\section{Entropy in information theory (maybe in appendix)}\label{sec:shannon}
The entropy notion that is most intricately connected with information is Claude E. Shannon’s entropy function, introduced in his seminal 1948 paper \emph{A Mathematical Theory of Communication} \cite{Sha48}. We consider finite sets $\{1,2,\dots,n\}$ of (mutually exclusive and exhaustive) \emph{alternatives} $i$, and probability distributions on these sets, which we denote by $\bm p = (p_i)_{i=1}^n = (p_1,p_2,\dots,p_n)$ (i.e.~$\forall i: 0\leq p_i\leq 1$ and $\sum_i p_i = 1$). Denote by $\mathcal P_n$ the set of probability distributions on $\{1,\dots,n\}$. The Shannon entropy $H$ is a function on from the set $\bigcup_n\mathcal P_n$ to $\R^+$. The entropy $H(\bm p)$ of a probability distribution $\bm p$ can be thought of as the expected amount of information necessary to specify the outcome when one of the alternatives is drawn according to $\bm p$. Alternatively, it is the amount of `missing information’, or `uncertainty’, if one of the alternatives is in fact the `true’ alternative, while all we know is the probability distribution.\footnote{Shannon’s interest was in the application in communication theory: a source sends out messages composed of words from a finite vocabulary. A receiver knows how the frequencies of the words are distributed but does not know the specific message that will be communicated.}

\subsection{Axiomatic derivation}
In search of such a function $H$, Shannon postulated that it should satisfy three axioms:
\begin{enumerate}
	\item $H$ should be continuous in the $p_i$.
	\item For uniform distributions, $H$ increases with the number of alternatives, since with more alternatives, it takes more information to pinpoint one of the alternatives/there is more uncertainty. Formally: if $m,n\in\N$ and \[ (p_i)_{i=1}^n = (1/n,\dots,1/n) \text{\quad and\quad} (q_j)_{j=1}^m = (1/m,\dots,1/m) \] and $m > n$, then $H(\bm q) > H(\bm p)$.
	\item $H$ is independent of the way the process of choosing a single alternative from the possibilities is divided into parts. Formally: Suppose the set of alternatives $(1,\dots, n)$ is partitioned into two groups $A$ and $B$, with probability $P_A = \sum_{i\in A} p_i$ and $P_B = \sum_{i\in B} p_i$ respectively. Denote $\bm P = (P_A, P_B)$. Then \[ H(\bm p) = H(\bm P) + P_A H(\{p_i/P_A : i\in A\}) + P_B H(\{p_i/P_B : i\in B\}). \] That is, the entropy involved in specifying one of the alternatives $i$ is equal to the weighted sum of the entropies involved in first specifying the group $A$ or $B$ and then specifying the individual alternative $i$.
\end{enumerate}

From these three axioms, Shannon proves \cite[Theorem~2]{Sha48} that $H$ must take the form
\begin{equation}\label{eq:shannon}
	H(\bm p) = -k \sum_{i=1}^n p_i \log p_i,
\end{equation}
where the logarithm can have any base and $k$ is a positive constant. Note that $H(\bm p) \geq 0$ for any probability distribution $\bm p$, and that $H(p) = 0$ iff there is only one alternative with non-zero probability; indeed, in that case there is no missing information. Moreover, in the space of probability distributions on $n$ alternatives, the unique distribution with maximal entropy is the uniform distribution $p_i = 1/n$. If $k=1$ and the logarithm has base 2, then the unit of $H$ is \emph{bit}.

\subsection{Interpretation of $H$ and the Noiseless Coding Theorem}\label{sec:shannon-interpretation}
The axioms of the entropy $H$ are based on the idea that it should represent the \emph{expected amount of missing information}. This is especially reflected in the third axiom. Considering Equation~(\ref{eq:shannon}), it might be tempting to view $-\log p_i$ as the \emph{actual} amount of missing information when $i$ is the true alternative. Indeed, this quantity is sometimes called the \emph{self-information} or \emph{information content} of the alternative $i$. However, this interpretation is not consistent; consider the case where there are only two alternatives, one with low probability $p_1$ and one with high probability $p_2$ (e.g.~an extremely biased coin toss). Then it takes only one bit to specify one of the alternatives, whereas $-\log p_1$ increases to infinity as $p_1$ approaches zero. In light of this, $-\log p_i$ is also called the \emph{surprise} of $i$.

The interpretation of $H$ becomes clearer in the context of Shannon’s \emph{Noiseless Coding Theorem}.\footnote{After proving Eq.~(\ref{eq:shannon}), Shannon notes that “this theorem, and the assumptions required for its proof, are in no way necessary for the present theory. It is given chiefly to provide a certain plausibility to some of our later definitions. The real justification of these definitions, however, will reside in their implications” \cite{Sha48}.} The setting is as follows. A source sends out messages composed of \emph{source words} $i$ in a vocabulary $\Sigma$ with probability $p_i$, and a \emph{code} $c$ encodes these messages by associating a finite binary sequence $c(i)$ of variable length (a \emph{codeword}) to each source word. Let $\mathcal C$ denote the set of all such codes $c: \Sigma \to \{0,1\}^*$, and $|c(i)|$ denote the length of the codeword for source word $i$, for $c\in\mathcal C$. Here $\{0,1\}^*$ is the set of finite binary sequences. Define the \emph{expected codeword length} by $L_c := \sum_i p_i |c(i)|$. The aim in communication theory is to find an optimal code, i.e.~a code with minimal expected codeword length. Let $L = \min\{ L_c : c\in\mathcal C \}$ be the expected codeword length of an optimal code. Then the Noiseless Coding Theorem states that
\[ H(\bm p) \leq L \leq H(\bm p) + 1. \]
Hence, $H(\bm p)$ can be seen as roughly equal to the \emph{least average number of bits required to communicate an alternative $i$, when the frequency of the alternatives is given by the probability distribution $\bm p$}. The \emph{Shannon-Fano code} is an optimal code that can easily be constructed from the probability distribution \cite{GrW08}.

The noiseless coding theorem also holds for probability distributions over countably infinite sets, as long as the Shannon entropy of the distribution $-k\sum_{i=1}^\infty p_i \log p_i$ converges \cite{GrW08}.

\todo{This is implied but not explained in GrW08. Is it true? Maybe useful: Baccetti and Visser, Infinite Shannon entropy}

We see that Shannon entropy can only be seen as a function of the probability distribution as a whole, and that it does not depend on the information inherent in the individual alternatives $i$ themselves. Shannon notes: “Messages have meaning, [however] the semantic aspects of communication are irrelevant to the engineering problem.” Also in physical systems, entropy should not be associated with the actual amount of information in the system, but always has to be viewed as a function of some probability distribution over the space of possible states of the system. Therefore there is no such thing as `the entropy’ of a system.

\subsection{Maybe: Relation to algorithmic information theory}
Still, there is a connection between the \emph{expected} algorithmic complexity of the alternatives of the distribution and its Shannon entropy. In the following theorem, we expand the set of alternatives from finite to countably infinite and consider the special case where the outcome space is given by the set of finite binary sequences $\{0,1\}^*$.
\todo{Maybe state Theorem 2.10 from \cite{GrW08}. But it doesn’t add much to the argument because it’s still only an expected value}

\subsection{Maybe: Continuous Shannon entropy}
Maybe introduce continuous Shannon entropy. Entropy can be made continuous, but then the connection with the notion of information is lost [Caticha 2008].


\section{Entropy and information in statistical mechanics}
Many different notions of entropy exist in physical theories. There are the multiple (phenomenological) thermodynamic approaches to entropy in the fashion of Clausius, Kelvin and Carnot, Boltzmann’s and Gibbs’ approaches to entropy in statistical mechanics, both of which come in coarse- and fine-grained versions, and von Neumann entropy in quantum mechanics. In the past century, also the entropy in black hole thermodynamics has shown to be important. All entropies are related in some way, and were in many cases constructed with the purpose of giving other explanations and derivations of the same notion.\footnote{The second law of thermodynamics was an important driving factor in the development of both statistical mechanics and black hole thermodynamics.} However, one must always be careful when equating two different notions of entropy. An important reason for this is that even when restricting oneself to only one of the above entropy concepts, there is no such thing as `the’ entropy of a physical system.

Instead, entropy is a property of the \emph{description} of the system: it depends on the available information, usually given in terms of macrostate variables. This is clear in the information theoretic context: the Shannon entropy is a function of the probability distribution, and has nothing to do with the inherent properties of the elements of the outcome space themselves, as discussed in the appendix/section~\ref{sec:shannon-interpretation}. In thermodynamics and statistical mechanics, the entropy is a function of the macrostate, which induces a probability distribution on the space of microstates, but what exactly is taken to be the macrostate and the microstate of a system differs from description to description. Edward~T.~Jaynes, who was an active researcher on the relation between information theory and statistical mechanics, interprets statistical mechanics as being a theory about our knowledge of the world, and not about the world itself \cite{FrW11, Jaynes1983 or Jaynes1957}.

\

Let us consider a possible way to relate entropy in statistical mechanics to information in the information-theoretic context. This connection is quite straightforward in the case of a coarse-grained entropy notion such as the coarse-grained Gibbs entropy. The finite-dimensional phase space is coarse-grained into cells of fixed volume. The macrostate is assumed given and induces a probability distribution on the countable set of microstate cells via the partition function. Let us denote the microstates with nonzero probability by $m\in M$, and their probability by $p_m$. (These probabilities are usually interpreted epistemically.) The coarse-grained Gibbs entropy is
\begin{equation}\label{eq:gibbs}
	S = -k_B \sum_{m\in M} p_m \ln p_m,
\end{equation}
where $k_B$ is the Boltzmann constant. If this sum converges (which is most often the case), then, noting the similarity between (\ref{eq:gibbs}) and the Shannon entropy (\ref{eq:shannon}), the Noiseless Coding Theorem amounts to the following:
\begin{quote}
	Given the thermodynamic state, if we let $\mathcal C$ be the set of codes $c : M \to \{0,1\}^*$ on the space of microstates, and denote by $L_c$ the expected codeword length of $c$, $L_c = \sum_m p_m |c(m)|$, then we have \[ S/(k_B\ln 2) < \min\{L_c : c\in\mathcal C\} < S/(k_B\ln 2) + 1. \]
\end{quote}
In section~\ref{sec:infinite-information} we will be concerned with the \emph{actual} amount of information `embodied’ in the system, that is, the minimal number of bits needed to describe its complete configuration. We see that the Gibbs entropy tells us little about this \emph{actual} amount: it only provides us with an \emph{expected value}. If the set of microstates with positive probability is countably infinite, then even an `optimal’ code might require arbitrarily many digits to describe the actual microstate.

\

Therefore, to be able to set an upper bound on this \emph{actual} minimal amount of information, we have to consider a macrostate where only a finite number of microstates have nonzero probability, i.e.~$|M| < \infty$. This is the case for Boltzmann’s coarse-grained entropy formulation, as in that case $E$ and $V$ are variables of the macrostate, so that the positions and momenta of all particles are bounded. Assuming equal a priori probability of microstates, the Boltzmann entropy $k_B\ln |M|$ is now proportional to the maximum Shannon entropy on $M$. However, the minimal amount of information of communicate the actual state of the system is now not a question of entropy anymore, but simply follows from the fact that there are only finitely many microstates: there is always a code $c:M\to\{0,1\}^*$ that is able to distinguish between the $|M|$ different microstates while using no more than $\log_2 |M|$ bits for each microstate.

Let $S$ be such a bounded system in the microcanonical ensemble, and let $M$ again be the set of coarse-grained microstates. We can make the reasonable assumption that
\begin{quote}
	there is a \emph{canonical} code $c: M\to\{0,1\}^*$ that represents each microstate in less than $\log_2 |M|$ bits,
\end{quote}
i.e.~one that is determined only by the system and a specified rule (e.g.~by lexicographically ordering the microstates expressed as $6N$-dimensional vectors), so that the function $c$ does not contain any new `information’ that we have to keep track of. If we also disregard the information necessary to translate a mathematical description into statements about physical reality, then we can conclude:
\begin{quote}
	The coarse-grained Boltzmann entropy $k_B\ln |M|$ gives (up to the multiplicative factor $k_B \ln 2$) an upper bound on the total number of bits needed to specify the coarse-grained microstate of the system, provided that its macrostate has already been specified.
\end{quote}
I must remark that a lot more can be said about the relation between entropy in statistical mechanics and information. See, for example, \textcite{tadaki2019}.



\section{Entropy and information in thermodynamics}
There are also a number of arguments from phenomenological thermodynamics\footnote{By arguments from phenomenological thermodynamics I mean arguments that describe thermodynamic phenomena without providing the underlying details of the system at the microscale.} that establish a connection between entropy and information, and information processing in particular. Especially Maxwell’s demon, Szilard’s engine and Landauer’s principle have sparked a historical and ongoing debate on this connection. Without going into this debate too deeply, I will outline Szilard’s argument and propose an alternative version that is relevant to the infinite precision of real numbers that we will discuss in section~\ref{sec:...}.

Szilard’s engine was proposed by Leo Szilard in 1929~\cite{sep-information-entropy} to provoke discussion on whether it can be used to violate the second law of thermodynamics. The engine consists of a box, in thermal contact with a heat bath of temperature $T$, containing a gas consisting of exactly one particle. A partition can be frictionlessly inserted into the centre of the box, dividing it into two separate volumes, and is also capable of sliding frictionlessly along the box in the horizontal direction. An intelligent being or ‘demon’ can insert the partition at a desired time point and couple it to a suspended weight via a cord and a pulley. If the demon knows in which half of the box the particle is at the moment of insertion (which can be described by one bit of information), it can attach the weight in such a way as to lift it using the pressure exerted by the particle on the partition. During this isothermal expansion of the single-particle gas, $k_B T\ln 2$ Joules of energy from the heat bath are converted into work. By repeating this process, the demon can extract arbitrarily much work from the heat bath.

This appears to violate the second law of thermodynamics. Szilard’s own analysis of this problem led to the conclusion that, for the second law to remain in effect, we have to assume that the process of coming to know the location of the particle comes with a minimum entropy cost of $k_B\ln 2$, regardless of the way that this information is obtained.

Others, notably Brillouin, have proposed generalised arguments that show that the acquisition of information through measurement requires energy dissipation of at least $k_B T \ln 2$ per bit. Landauer, on the other hand, argued that the \emph{erasure} of a bit of information is what requires the energy dissipation.

\

It is also useful to consider what happens when it is possible to know the location of a particle with arbitrary precision. This information can be expressed in terms of bits and therefore Brillouin’s and Landauer’s principles may be applied, but in anticipation of section~\ref{sec:...} an argument is desirable that does not depend on the binary representation of this information. This can be achieved by slightly modifying Szilard’s engine. In this modification, two partitions can be inserted into the box, dividing it into three regions. Suppose the demon knows the position of the particle with an accuracy of $\e L$, where $L$ is the length of the box and $0 < \e < 1$. Then it can place the two partitions around the particle, at a distance of $\e L$. By attaching pulleys to both partitions and allowing the single-particle gas to expand to its original volume, now an energy of $-k_B T\ln\e$ is extracted from the heat bath and converted into work.\footnote{The ideal gas law gives $P = k_B T / V$ for the pressure of the particle exerted on the partitions, so the total work performed is $\int_{V_i}^{V_f} P\dif V = k_B T \ln(V_f/V_i) = -k_B T \ln\e$.} This decreases the entropy of the system by $-k_B\ln\e$. If the second law cannot be violated, we conclude that acquiring the information about the location of the particle must have required an entropy cost of at least $-k_B\ln\e$. As the accuracy in the location of the particle increases, $\e$ approaches zero and the entropy cost diverges to infinity.


\section{The Bekenstein bound}
The Bekenstein bound is an upper bound on the entropy-to-energy ratio of a bounded system. There are several heuristic arguments in favour of the bound, and in 2008 a more rigorous proof was given by Horacio Casini in the context of quantum field theory. The domain of applicability of the bound remains a subject of debate, in part because of its ambiguous formulation \cite{page2018}. I will not go into the several derivations here but briefly present an argument for weakly self-gravitating systems based on black hole thermodynamics from \textcite{bekenstein1981}. Suppose the system, which is assumed to be enclosed in a sphere of radius $R$ and to have energy content $E$ and entropy $S$, is lowered into a black hole with a mass much larger than the system's mass. Then the system and its entropy disappear from view, but the entropy of the black hole increases. It is a result of black hole thermodynamics that in the process of dropping such a system into a black hole, the surface area of the hole increases by at least $\frac{8\pi GRE}{c^4}$, and that the process can be arranged such that this bound is attained. The black hole entropy being given by $\frac{c^3A}{4G\hbar}$, with $A$ the surface area of the black hole, we see that the entropy of the hole increases by $\frac{2\pi RE}{\hbar c}$. By the (generalised) second law of thermodynamics, the entropy of the system plus the black hole cannot decrease, so we must have $-S + \frac{2\pi RE}{\hbar c} \geq 0$, or equivalently
\begin{equation}\label{eq:bekenstein}
	S \leq \frac{2\pi RE}{\hbar c}.
\end{equation}

This is the Bekenstein bound. We will discuss the implications of this bound on the information contained in a physical system in section~\ref{sec:...}.

